Learning to Generate Better Than Your LLM

Reinforcement learning (RL) has emerged as a powerful paradigm for fine-tuning Large Language Models (LLMs) for text generation. In particular, recent LLMs such as ChatGPT and GPT-4 can engage in fluent conversations with users after finetuning with RL. Capitalizing on key properties of text generation, we seek to investigate RL algorithms beyond general purpose algorithms like Proximal Policy Optimization (PPO). In particular, we extend RL algorithms to allow them to interact with a dynamic black-box guide LLM and propose RL with guided feedback (RLGF), a suite of RL algorithms for LLM fine-tuning. We provide two ways for the guide LLM to interact with the LLM to be optimized for maximizing rewards. The guide LLM can generate text which serves as additional starting states for the RL optimization procedure. The guide LLM can also be used to complete the partial sentences generated by the LLM that is being optimized, treating the guide LLM as an expert to imitate and surpass eventually. We experiment on the IMDB positive sentiment, CommonGen, and TL;DR summarization tasks. We show that our RL algorithms achieve higher performance than supervised learning (SL) and the RL baseline PPO, demonstrating the benefit of interaction with the guide LLM. On both CommonGen and TL;DR, we not only outperform our SL baselines but also improve upon PPO across a variety of metrics beyond the one we optimized for. Our code can be found at https://github.com/Cornell-RL/tril.

==> intro.tex <==
Large Language Models (LLMs) have become very capable in various real-world applications ranging from being able to answer open-ended questions on numerous topics~\citep{zhang2022greaselm}, write articles from short descriptions~\citep{goyal2022news}, generate code~\citep{Githubcopilot}, follow robot commands~\citep{huanginner}, solve puzzles~\citep{bubeck2023sparks}, and even showcased as assistive models for education~\citep{KhanAcademy} and healthcare~\citep{lee2023benefits}. 




However, using supervised learning (SL) to train LLMs presents a challenging metric mismatch \citep{wiseman2016sequence} between the training and testing regimes. The metric mismatch arises from the training metric being the log-loss while the testing metrics are task-specific such as BLEU or user satisfaction rating. This discrepancy is magnified when fine-tuning LLMs on downstream tasks where the main goal is not just producing fluent text but also being proficient at solving the specific task. \looseness=-1

Reinforcement Learning (RL) by definition address this metric mismatch by directly optimizing the metrics through reward feedback. %
Recently, OpenAI fine-tuned LLMs with RL from human feedback (RLHF) to better align LLMs to human intentions, leading to the great success of ChatGPT \citep{chatgpt}.  Recently, GRUE benchmark \citep{ramamurthy2022rl4lm} systematically studied RL versus SL when finetuning LLMs on downstream tasks with pre-defined rewards. GRUE's preliminary results demonstrate the benefit of RL when finetuning LLMs, leading to the release of popular codebases such as RL4LMs \citep{ramamurthy2022rl4lm}, TRLx \citep{trlx} and AlpacaFarm \citep{dubois2023alpacafarm}, that enables RL for language models. However, ChatGPT, RL4LMs, TRLX, and AlpacaFarm all use vanilla policy gradient methods known to be sample inefficient and sensitive to local minima due to the combinatorially large search space of natural language generation \citep{ramamurthy2022rl4lm}. \looseness=-1

In this work, we focus on more efficient ways of fine-tuning LLMs on downstream tasks with predefined rewards.
Our approach is motivated by prior work on Imitation Learning (IL) for structured prediction which often leverages an existing guide policy (not necessarily an optimal policy) to reduce the search space for more efficient and optimal learning. Our key observation is that since modern LLMs exhibit impressive general language capabilities, they can serve as guide policies to improve the RL procedure. %
Our framework, which we call, \emph{RL with guided feedback} ($\framework$), integrates a guide policy into a policy gradient framework. %
The guide policy can provide reasonable but sub-optimal predictions for downstream tasks which our framework can then leverage to learn a near-optimal strategy. 
We introduce novel algorithms for fine-tuning LLMs using our $\framework$ framework while capturing various existing IL for structured prediction and RL algorithms. 

We evaluate on three tasks. The first is IMDB where the goal is to generate a positive and fluent review given an initial context. The second is CommonGen where the goal is to write a fluent text that uses a given set of words. Finally, we test on TL;DR, a summarization task with human preferences. For all tasks, we find evidence of metric mismatch from SL-based fine-tuning approaches and show that RL-based methods which utilize reward signals outperforms on the task metric. We then demonstrate \framework{} outperforming PPO on reward, fluency, as well as automated lexical metrics such as Rouge. Finally, we investigate how various baselines and \framework{} algorithms balance the inherent tradeoff between reward optimization and the KL constraint in the RLHF objective.
















